Parallel algorithms for mining of frequent itemsets

In the recent decade companies started collecting of large amount of data. Without a proper analyse, the data are usually useless. The field of analysing the data is called data mining. Unfortunately, the amount of data is quite large: the data do not fit into main memory and the processing time can become quite huge. Therefore, we need parallel data mining algorithms. One of the popular and important data mining algorithm is the algorithm for generation of so called frequent itemsets. The problem of mining of frequent itemsets can be explained on the following example: customers goes in a store put into theirs baskets some goods; the owner of the store collects the baskets and wants to know the set of goods that are bought together in at least p% of the baskets. Currently, the sequential algorithms for mining of frequent itemsets are quite good in the means of performance. However, the parallel algorithms for mining of frequent itemsets still do not achieve good speedup. In this thesis, we develop a parallel method for mining of frequent itemsets that can be used for an arbitrary depth first search sequential algorithms on a distributed memory parallel computer. Our method achieves speedup of ~ 6 on 10 processors. The method is based on an approximate estimation of processor load from a database sample - however it always computes the set of frequent itemsets from the whole database. In this thesis, we show a theory underlying our method and show the performance of the estimation process.

==> 06_dataset_generators.tex <==
\chapter{The assessment of the IBM generator}\label{chap:ibm-gener-assesment}


Due to the lack of real databases, we have generated large data sets
using the IBM data generator \cite{agrawal94fast}. While making
hundreds of experiment with the parallel FIMI algorithms, we have
observed that the experiments with our parallel algorithm behaves very
differently for different parameters of the IBM generator and for the
real databases.


The most important databases, we should use for measurement, are the real
databases. Unfortunately, we are not able to use the real databases for
experiments with the parallel algorithms, because they are too small.

In this section, we will describe the most important differences
between the databases generated by the IBM generator and the real
databases. As a real databases, we consider the databases dowloaded
from the internet \cite{fimi03}.


\section{The IBM database generator}

The IBM random database generator \cite{agrawal94fast} creates a
database of items bought by a customer in a retail shop. The generator
mimics the behavior of the consumers in a supermarket. The generator
has the following parameters:

\begin{enumerate}
\item $N$, the number of items.
\item $|L|$, the number of potentionaly frequent itemsets.
\item $E(|I|)$, the average size of the maximal potentionally frequent itemsets
\item $E(|T|)$, the average size of the transaction.
\item $|D|$, the size of the database.
\end{enumerate}

The generation of the database is done in two steps: 1) the
potentionally frequent itemsets are generated; 2) the database is created
from the generated potentionally frequent itemsets.

The potentionally frequent itemsets are generated in the following
way: the number of frequent itemsets is set to $|L|$. The length of
the potentionally frequent itemset is generated from the Poisson
distribution with mean $E(|I|)$. The items in the first frequent
itemset are picked randomly. In subsequent frequent itemsets, some
fraction of the items are picked from previous transaction using the
exponential distribution with mean $0.5$. The rest of the items are
picked randomly. Each itemset in $L$ is assigned a weight that
corresponds to the probability that an itemset is chosen. The weight
is picked from the exponential distribution with mean $1.0$. The
weights are normalized, so they sum to $1$. Each potentionally
frequent itemset is also assigned a corruption level $c\in\lcint
0,1\rcint$.

From the potentionally frequent itemsets $L$, we generate $\db$ in the
following way: first, the size of the transaction is picked from the
Poisson distribution with mean equal to $E(|T|)$. Then a set of
potentionally frequent itemsets is picked from $L$.  Each frequent
itemset is chosen from $L$ randomly with probability proportional to
the weight of the frequent itemsets in $L$. If the frequent itemsets
do not fit into the transaction, in half of the cases the last
frequent itemset is put into the transaction, and the itemset is moved
to the next transaction in the rest of the cases. To model the fact
that not all items from a frequent itemset are put into the
transaction, a uniform random numbers from $\lcint 0,1\rcint$ are
generated and the items are dropped until the random numbers are less
then the corruption level $c$.



\section{The other database generators}


There are other approaches to generate artificial databases.  Ramesh,
Zaki and Maniatty \cite{zaki05gener} presents an approach that takes
$k$ sets of maximal itemsets $\mfi_i$ satisfying the \emph{containment
  property}, i.e. $\mfi_1\sqsubseteq\mfi_2$ if and only if for each
$m_1\in \mfi_1$ there exists $m_2\in \mfi_2$ such that $m_1\subseteq
m_2$, and generates a database that has $\mfi_i$ as the MFIs at
certain support level.


The containment property \emph{assures} that there are no other MFIs
generated from the database, for proof see \cite{zaki05gener}. The
support of the MFIs is chosen by the generator and for the supports of
$m_1\in\mfi_i, m_2\in\mfi_j$ holds that $\supp(m_1) \geq
\supp(m_2)$. The generator generates the database by repeating the
itemsets $\mfi_i$. The authors of \cite{zaki05gener} have noticed that
this procedure can generate a very large databases of size
$O(n\cdot\prod_{i=i}^n |\mfi_i|)$. As claimed there, the generation
procedure is simple and sensitive to the initial sets of MFIs.


The Cooper and Zito generator \cite{zito07gener} is trying to create
correlations among the items by choosing part of the items from
previous transactions and part of the new items similarily as the IBM
generator while generating candidate itemsets. The generator combines:
1) items from a previous transaction and new items; 2) items from an
old transactions.  The Cooper and Zito generator takes the itemsets
from previous transactions at random and combines them with new items
or from previous transactions at random.  By a similar argument as for
the IBM generator, we conjecture that the Cooper and Zito generator
generates database with extensions of CI with size $>2$ with very
small probability.

The problem with the generator made by Ramesh, Zaki and Maniatty
\cite{zaki05gener} is that the generator generates unrealistic
databases by repeating itemsets.





\section{The database characteristics}


For the development of efficient parallel algorithms, we need real
large databases, usable for the measurements of the parallel
speedup. Therefore, we have generated the databases using the IBM
generator.  While working on parallel algorithms for mining of FIs, we
have observed differences between the data generated by the IBM data
generator and the \emph{real databases}. To compare the data generated
by the IBM generator and the real databases, we need to have some
database characteristics. These differences are demonstrated using
several database characteristics that are derived from properties
important for the efficiency of the sequential and parallel algorithms
for mining of FIs.



The database characteristics are divided into two groups: 1) the
distribution of parameters of generated objects; 2) the structure of
the set of all FIs. The two groups of characteristics complement each
other.



\subsection{CI extension characteristics}\label{sec:cistat}

A DFS algorithm uses the prefix-based equivalence classes to
recursively partition $\allfi$. A DFS algorithm need to view the set
$\baseset$ as an ordered set in order to construct the prefix-based
equivalence classes. Each prefix-based class with a prefix
$\itsetprefix$ has some extensions $\prefixext$.

A DFS algorithm (like Eclat or FPGrowth) can use $\tcover\circ \bcover$
for optimization a DFS algorithm, i.e. a DFS algorithm can extend
the prefix $\itsetprefix$ using the extensions $\isetW = \{\ext_i |
\ext_i\in\prefixext, \supp(\itsetprefix \cup \{ \ext_i \} = \supp(
\itsetprefix) \}$ without the computation of supports of the sets
$\itsetprefix\cup\isetU, \isetU \subseteq \isetW$. Therefore, using
the extensions $\isetW$ we save $O(2^{|\isetW|})$
computations of support. It would seem that $\tcover\circ \bcover$
computes the set of all CIs, i.e. every set $\itsetprefix\cup\isetW$
is a closed itemset. But, $\itsetprefix\cup\isetW$ need not to be
CI. Every CI appears exactly once as the union
$\itsetprefix\cup\isetW$. The details of the Eclat algorithm, the
FPGrowth algorithm and its optimizations can be found in Sections
\ref{sec:fpgrowth-algorithm}, \ref{sec:eclat-algorithm}, and
\ref{sec:dfs-optimizations}.

% $\tcover\circ \cover$
Our goal is to estimate the amount of optimizations as described above
made by a DFS algorithm. For this, we use the modified Eclat
algorithm. Based on the discussion of the optimizations made by a DFS
algorithm we have created the two following characteristics:

\emph{The size of the extension: } This characteristic is a histogram
of $|\isetW|$. On the x-axis is $|\isetW|$ and on the y-axis is the
number of extensions. 


\emph{The size of closed itemsets and the size of the extension:} to
see the characteristics from the previous paragraph in a more detail,
we also show a histogram of $|\itsetprefix\cup\isetW|$ for every size
$|\isetW|$. Therefore, we have as many histograms as the sizes
$|\isetW|$.

On the x-axis is $|\itsetprefix\cup\isetW|$ and on the y-axis is the
frequency. Each line corresponds to $|\isetW|$. 


\if0
\begin{figure*}[!p]
\vbox{\hskip-1.0cm\hbox{
\scalebox{0.5}{\includegraphics[type=\picext,ext=.\picext,read=.\picext]{pics/db_chars/mushroom-0.1.eclat_ext_stat}}
\scalebox{0.5}{\includegraphics[type=\picext,ext=.\picext,read=.\picext]{pics/db_chars/mushroom-0.1.ci_stat}}
}}
\caption{The \texttt{mushroom} database, $\minsupp=0.14$}
\end{figure*}

\begin{figure*}[!p]
\vbox{\hskip-1.0cm\hbox{
\scalebox{0.5}{\includegraphics[type=\picext,ext=.\picext,read=.\picext]{pics/db_chars/T200I0.1-0.14.eclat_ext_stat}}
\scalebox{0.5}{\includegraphics[type=\picext,ext=.\picext,read=.\picext]{pics/db_chars/T200I0.1-0.14.ci_stat}}
}}
\caption{The IBM-generated \texttt{T200I0.1} database, $\minsupp=0.14$}
\end{figure*}
\clearpage
\fi



\subsection{The FI characteristics}\label{sec:fistat}

Another important characteristic is the distribution of the supports and
lengths of FIs. The FI characteristic is displayed as a map (a 2D
histogram). The level of grey at each point shows the number of FIs
with particular parameters. Because the number of FIs can differ by
orders of magnitude, the level of grey is displayed in $\log_{10}$
scale. Therefore, the level of grey compares the orders of the number
of FIs.

The histogram has the lengths of a FIs on the X axis and the supports
of FIs on the Y axis. Because the support is a real value, we have
divided the interval $\langle 0,1 \rangle$ on $n=1000$ subintervals
$\langle i\cdot \frac{1}{n}, (i+1)\cdot \frac{1}{n} \rangle$ for
$i=0,1,\ldots n-1$.

To construct the map we have used the modified Eclat algorithm. The
Eclat algorithm computes all FIs and it increments the counter
associated with each combination of support and length.


\subsection{The maximal frequent itemset characteristics}\label{sec:mfistat}

We have observed that the parameters of MFIs are important. We have
computed the lengths of MFIs for several values of minimal
supports. For each value of support we can draw a histogram of lengths
(on the X axis) versus the number (on the Y axis) of MFIs with
particular length. The histograms are displayed in a single map (a 2D
histogram). The level of grey at each point corresponds to the number
of MFIs with particular length and support. Because the number of MFIs
can be quite large we have displayed them in the $\log_{10}$ scale.

The graph is constructed similarly as the graphs from
\secref{sec:fistat}.  Each row in the graph corresponds to a single
run of an algorithm for mining of MFIs with particular value of
minimal support. The level of grey of each point corresponds to the
number of MFIs for particular value of length and minimal support.


There is a difference between the FI and MFI characteristic. Single
graph with the FI characteristic is computed for single value of minimal
support. The graph with the MFI characteristic is computed for many
values of minimal support.

The motivation behind the characteristic is the bad speedup of the
static load-balancing for parallel mining of FIs for particular
parameters of the IBM generator. The MFIs influence the structure of
the set of all FIs. For example, if we have $\approx 500000$ MFIs with
small intersections and we sample $\approx 40000$ samples of FIs the
sample does not represent well the set of all FIs. The consequence of
this is the bad estimation of sizes of particular prefix-based classes
and bad speedup of the parallel algorithm for mining of FIs.

To compute the MFI characteristic, we have used a modified
\emph{fpmax*} algorithm \cite{grahne03fpmax}.



\subsection{The Pagerank distribution function}\label{sec:pagerankstat}

It is possible to characterize the MFIs using the connectivity of the
directed graph of MFIs. Let $\nodes$ is the set of nodes, node
$\node_i$ corresponds to MFI $\smfi_i$ and $\edges =
\{(\node_i,\node_j)\}$ be a set of edges of a graph $G =
(\nodes,\edges)$. The edge $(\node_i,\node_j)$ is present in the graph
if $\frac{ |\smfi_i\cap\smfi_j| }{ |\smfi_i| } \geq
min\_edge\_weight$, where $min\_edge\_weight$ is a parameter of the
computation.



The number of MFIs can be quite large, ranging from $\approx 10000$ to
$\approx 500000$. Consequently, computing the adjacency matrix of the
whole graph is quite time consuming.  Although the matrix is sparse,
it can consume significant amount of memory. Therefore, we have
decided to uniformly sample the MFIs and compute the pagerank on a
subset of MFIs of manageable size.


To measure the connectivity, we have used a modified \emph{pagerank}
algorithm \cite{page99pagerank}. The original pagerank values are
computed from the following equation:

$$\pagerank(\node_i) = (1-d) + d\cdot\sum_{\node_j\in N(\node_i)}\pagerank(\node_j)\cdot w_{ji}$$

\noindent where $N(\node_i)$ is the set of successors of the node
$\node_i$ and $w_{ji}=1/L(\node_j)$, where $L(\node_j)$ is the number
of \emph{outgoing} edges of $\node_j$ and $d$ is the \emph{damping
  factor}. We have modified this equation and redefined $w_{ij}$ to be
the weight of the link from $\node_i$ to $\node_j$ using the formula
$w_{ij} = \frac{ |\smfi_i \cap \smfi_j| }{ |\smfi_i|}$.


The \emph{pagerank} of nodes ${\cal V}$ is displayed as the
\emph{distribution function} $D(x)=|\{ v_i\in{\cal V} | \pagerank(v_i)
\leq x \}|/|{\cal V}|$, i.e. the relative number of nodes with the
pagerank value at most $x$. For example if there is a point on the
curve with coordinates $(x,y)=(0.5,0.4)$ it means that $\approx 40\%$
of the nodes have pagerank value at most $0.5$.

The motivation behind the pagerank characteristic is to measure the
level of clustering of MFIs into groups of similar MFIs.


\section{Experimental comparison of real and IBM generated databases}

We have compared the characteristics of the IBM generated databases
with high ($1000$), low ($100$) number of items, and the real
databases. We have generated the databases using the IBM generator with
the following parameters: $100$ patterns with average pattern length
$20$, the transaction length $50$, and $200000$ transactions. We will
denote the IBM generated database with $100$ items as \texttt{T200I0.1}
and the IBM generated database with $1000$ items as
\texttt{T200I1}. The real databases were downloaded from \cite{fimi03}.

In this Section, we compare the database characteristics. We have
choosen the most typical results from our experiments that clearly
show the differences among the databases. From our experiments follows
that the \texttt{T200I0.1} has characteristics much closer to the real
databases then the \texttt{T200I1}.



\textbf{The CI characteristics:} The CI characteristics shows the
amount of optimizations of a DFS algorithm for mining of FIs that
uses the compound projection $\tcover \circ \bcover$. The graphs on
Figure \ref{ci-stat-t200} clearly shows that the IBM generated
databases do not contain extensions longer then $1$. Generally, the
number of extensions of size $2,3$ is very small for the IBM generated
data.  The Figure \ref{ci-stat-mushroom} shows a typical graphs for
real databases: the fraction of extensions of size $>3$ is quite large.


\textbf{The MFI characteristics:} the graphs on the Picture
\ref{mfi-stat} show the possible combinations of support(y-axis) and
length(x-axis) of MFIs. The picture shows the graphs for the three
selected databases. The area corresponding to the possible
combinations of support and length is more compact on the left graph
and on the right graph. These two graphs corresponds to the
\texttt{T200I0.1} (left) and to the real database \texttt{connect}
(right).

The middle graph shows the characteristic for the \texttt{T200I1}. The
area corresponding to the possible combinations of length and support
has gaps. For example for the support $0.09$ there are MFIs of length
$1,2,3,4,5$ then a gap and then MFIs of length $15$. The graphs for
the real databases and the \texttt{T200I0.1} does not have such gaps.


\textbf{The Pagerank characteristics:} the distribution of the
Pagerank values was computed with the damping factor $0.8$ and
$min\_edge\_weight=0.6$. The pagerank is computed in iterations. Each
iteration makes the computation more precise. The algorithm computes
the difference of the pagerank values from the current iteration and
the previous iteration. When the difference is less then $0.01$ we
stop the computation.

The graphs shows the distribution function of the Pagerank values. The
distribution function helps to display the clusters of values. The
clusters of values are displayed as the steep parts of the curves. The
graphs of the characteristic is show on Picture \ref{pagerank-graphs}.


The graphs clearly show the difference between the \texttt{T200I0.1},
the real databases and the \texttt{T200I1}. The \texttt{T200I1} database
has $2$-$3$ clusters of values close to $1-d$, where $d=0.2$ is the
damping factor. The \texttt{connect} database has many small clusters
of values $>0.8$. The \texttt{T200I0.1} has larger cluster of values
close to $0.2$ and many clusters of values $>0.8$.


\textbf{The connection between the MFI and the Pagerank
  characteristics:} maybe there is a connection between the MFI and
the Pagerank characteristic. The graphs on the Figures \ref{mfi-stat},
\ref{pagerank-graphs}, and \ref{mfi-intersections-ibm} show the
connection between the Pagerank distribution and the MFI
characteristic. The graph \ref{mfi-stat} shows that the
\texttt{T200I1} database has large number of small MFIs, i.e. MFIs of
length $1$-$5$. Additionally the graphs on Figure
\ref{mfi-intersections-ibm} show that two MFIs computed from
\texttt{T200I1} have usually very small intersection size ($<3$). Our
hypothesis is that the cluster of the Pagerank values values of
\texttt{T200I1} and the properties of the graphs in \ref{mfi-stat} and
\ref{mfi-intersections-ibm} may be related. The reason for the large
clusters of pagerank values close to $1-d=0.2$ can be the fact the
intersections are small and do not form clusters.


\textbf{The FI characteristics:} (opsane z clanku, asi nutno
preformulovat aby to nebylo stejne) The graphs in \figref{fi-stat-fig}
show that the lengths of the FIs grow with decreasing support
differently for the IBM generated and real databases.

For the IBM generated databases $I=1$, there are several intervals of
support with long FIs, while for the intermediate interval of supports
the long FIs disappear. This pattern is present only in a very small
part of the graph for the for $I=0.1$.

There is a difference between the \texttt{T200I0.1} and the real
databases. The lengths of FIs for \texttt{T200I0.1} grow with
decreasing support much more for smaller values of support than for
the real databases.



\textbf{Connection between the FI and the MFI graphs:} (opsane z
clanku, asi nutno preformulovat aby to nebylo stejne) First note, that
the MFIs determine the FIs. Long MFIs disappear at certain support
level (e.g. $\minsupp=0.11$ and the length $16$ for the
\texttt{T200I1} database). Because the FIs are subsets of MFIs, there
are no long MFIs then FIs also cannot be long.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% CI CHARACTERISTICS



\begin{figure*}[!p]
\centering
\hbox{
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/mushroom-0.1.eclat_ext_stat}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/mushroom-0.1.ci_stat}}
}
\caption[Typical CI characteristic measured on real database]{The typical CI statistics, measured on the \emph{real
    database} \texttt{mushroom} database. The  graphs are
  described in the Section \ref{sec:cistat}}
\label{ci-stat-mushroom}
\end{figure*}



\begin{figure*}[!p]
\centering
\hbox{
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I0.1-0.14.eclat_ext_stat}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I0.1-0.14.ci_stat}}
}
\caption[Typical CI characteristic measured on IBM database]{The CI statistics measured on the \emph{IBM-generated}
  \texttt{T200I0.1} database with support 0.14. The graphs are
  described in the Section \ref{sec:cistat}. The graphs for the
  \texttt{T200I1} are similar.}
\label{ci-stat-t200}
\end{figure*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure*}[!p]
\centering
\hbox{
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I0.1.mfistat}}
\rotatebox{90}{\scalebox{0.345}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I1.mfistat}}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/connect.mfistat}}
}
\caption[Typical MFI characteristic.]{A typical database MFI characteristics. From left to right: 1)
  the \texttt{T200I0.1} database; 2) \texttt{T200I1} database; 3) the
  \texttt{connect} database. The graphs are described in the
  \secref{sec:mfistat}.}
\label{mfi-stat}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[!p]
\centering
\hbox{
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I0.1.pagerank}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I1.pagerank}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/pumsb.pagerank}}
}
\caption[Distribution of the pagerank values.]{The distribution of the pagerank values. From left to right:
  1) \emph{IBM generated} \texttt{T200I0.1}; 2) the \texttt{T200I1};
  3) the \texttt{pumsb} databases. The graphs are described in the
  \secref{sec:pagerankstat}.}
\label{pagerank-graphs}
\end{figure*}




\begin{figure*}[!p]
\centering
\hbox{
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I0.1-0.11-D0.8-EPS0.001-INTPCT0.6.weighted_pagerank.intersections}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I1-0.09-D0.8-EPS0.001-INTPCT0.6.weighted_pagerank.intersections}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/connect-0.7-D0.8-EPS0.001-INTPCT0.6.weighted_pagerank.intersections}}
}

\caption[Histogram of the sizes of the intersections of pairs of
  MFIs]{The histogram of the intersections of pairs of MFIs. From left
  to right: 1) the \emph{IBM generated} \texttt{T200I0.1}
  ($\minsupp=0.11$); 2) the \texttt{T200I1} ($\minsupp=0.09$) 3) the
  \texttt{connect} ($\minsupp=0.7$). }
\label{mfi-intersections-ibm}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure*}[!p]
\centering
\hbox{
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I0.1-0.12.fistat}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/T200I1-0.03.fistat}}
\scalebox{0.3}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/connect-0.1.fistat}}
}
\caption[Typical FI characteristic.]{The FI characteristic. From left to right: 1) the
  \texttt{T200I0.1} database; 2) the \texttt{T200I1} database; 3) a
  typical real database FI characteristic, measured on the
  \texttt{connect} database. The graphs are described in the
  \secref{sec:fistat}.}
\label{fi-stat-fig}
\end{figure*}












\if0
\begin{figure*}[!p]\label{fistat-t200}
\vbox{\hskip-1.0cm\hbox{
\scalebox{0.5}{\includegraphics[type=\picext,ext=.\picext,read=.\picext]{pics/db_chars/fistat/T200I0.1-0.12.fistat}}
\scalebox{0.5}{\includegraphics[type=\picext,ext=.\picext,read=.\picext]{pics/db_chars/fistat/T200I1-0.03.fistat}}
}}
\caption{The IBM-generated \texttt{T200I0.1}($\minsupp=0.12$) database
  and \texttt{T200I1}($\minsupp=0.03$). NENI JASNE PROC SROVNAVAM
  ZROVNA TY DVA SUPPORTY}
\end{figure*}


\begin{figure*}[!p]\label{fistat-connect}
\centering
\vbox{\hskip-1.0cm\hbox{
\scalebox{0.5}{\includegraphics[type=\picext,ext=.\picext,read=.\picext]{pics/db_chars/fistat/connect-0.1.fistat}}
%\scalebox{0.5}{\includegraphics[type=\picext,ext=.\picext,read=.\picext]{pics/db_chars/fistat/T200I1-0.03.fistat}}
}}
\caption{The \texttt{connect} database - a typical picture of a real
  database}
\end{figure*}



\begin{figure*}[!p]
%\moveleft2cm 
\vbox{\hskip-1.5cm\hbox{
\scalebox{0.5}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/mfistat/T200I0.1.mfistat}}
\scalebox{0.5}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/mfistat/T200I1.mfistat}}
}}
\caption{A typical IBM generated database characteristics. On the left
  is the \texttt{T200I0.1} database, on the right is the
  \texttt{T200I1} database. The graphs are described in the
  \secref{mfi-hist-stat}.}
\label{mfi-stat-ibmgen}
\end{figure*}


\begin{figure*}[!p]
\centering
\vbox{\hskip-1.5cm\hbox{
\scalebox{0.5}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/mfistat/connect.mfistat}}
}}
\caption{A typical real database MFI characteristics, measured on the
  \texttt{connect} database. The graphs are described in the
  \secref{mfi-hist-stat}.}
\label{fi-stat-realdb}
\end{figure*}



\begin{figure*}[!p]
%\moveleft2cm 
\vbox{\hskip-1.5cm\hbox{
\scalebox{0.5}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/pagerank/T200I0.1.pagerank}}
\scalebox{0.5}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/pagerank/T200I1.pagerank}}
}}
\caption{The distribution of the pagerank values, measured on the
  \emph{IBM generated} \texttt{T100I0.1} (left) and the
  \texttt{T200I1} (right). The graphs are described in the
  \secref{mfi-connect-stat}.}
\label{mfi-connect-stat-ibm}
\end{figure*}


\begin{figure*}[!p]
%\moveleft2cm 
\centering
\scalebox{0.5}{\includegraphics[type=pdf,ext=.pdf,read=.pdf]{pics/db_chars/pagerank/pumsb.pagerank}}
\caption{A typical \emph{real} database characteristics measured on
  the \texttt{pumsb} database. The graphs are described in the
  \secref{fi-stat}.}
\label{mfi-connect-stat-real}
\end{figure*}

\fi

\clearpage


==> Makefile <==
TEXFILES=00_symbols.tex \
        00_abstract.tex \
        00_dedication.tex \
	00_acknowledgement.tex \
	01_math_found.tex \
	02_problem_definition.tex \
	03_contribution.tex \
	03_exist_seq_alg.tex \
	04_exist_par_alg.tex \
	05_approx_counting.tex \
        05_parallel_mfi.tex \
	05_ppmfi.tex \
	06_experiment_eval.tex \
	06_exec_eclat.tex \
	06_db_repl.tex \
	06_dataset_generators.tex \
	appendix_sequential_algo.tex \
	appendix_discrete_distributions.tex \
	phd_thesis.tex \
	myshortcuts.sty \
	papers.bib \
	07_future_work.tex \
	abbreviations.tex \
	lattice_mfiparallel.mps \
	sample_mfis.mps \
	lattice_dfstree_plain.mps \
	lattice_dfstree_pbec.mps \
	refereed_papers.bbl \
	unrefereed_papers.bbl

phd_thesis.pdf: allpapers.bbl $(TEXFILES) tables/avg_speedups/*.ltx.bold
	pdflatex phd_thesis.tex
	bibtex phd_thesis
	pdflatex phd_thesis.tex
	pdflatex phd_thesis.tex

phd_thesis.dvi: phd_thesis.tex
	latex phd_thesis.tex
	bibtex phd_thesis
	latex phd_thesis.tex
	latex phd_thesis.tex

%.mps: mpost/lattice.mp mpost/sample.mp
	make -C mpost all

#mpost/lattice.mp mpost/sample.mp
mpost: mpost/lattice.mp mpost/sample.mp
	make -C mpost all

phd_thesis.ps: phd_thesis.pdf
	pdftops phd_thesis.pdf phd_thesis.ps

phd_thesis-2on1.ps: phd_thesis.ps
	psnup -2 phd_thesis.ps phd_thesis-2on1.ps

ps: phd_thesis.ps

ps21: phd_thesis-2on1.ps

pdf21: phd_thesis-2on1.pdf

phd_thesis-2on1.pdf: phd_thesis.pdf
	pdfnup --nup 2x1 --outfile phd_thesis-2on1.pdf phd_thesis.pdf

clean:
	rm -rf *.dvi phd_thesis.pdf *.aux *log *blg *~ phd_thesis*.ps *.loa *.lof *.lot *.toc
# *.bbl
#*.mps
#	@- make -C mpost clean

convertps:
	./convert_to_pdf.sh pics/dbrepl


allpapers.bbl: allpapers.tex mypapers.bib
	pdflatex allpapers.tex
	bibtex allpapers.aux
	pdflatex allpapers.tex

.PHONY: mpost clean

==> tables/avg_speedup_fimipar.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40   & \textbf{1.481} & \textbf{2.160} & \textbf{2.809} &  2.073          & 1.853          &    1.563 \\ \hline 
T500I0.1P50PL20TL40   & \textbf{1.636} & \textbf{2.633} & \textbf{3.506} &  \textbf{5.028} & 5.511          &    6.304 \\ \hline 
T500I0.4P250PL20TL80  & \textbf{1.039} & \textbf{1.954} & \textbf{2.726} &  \textbf{3.422} & \textbf{3.945} &    \textbf{4.010} \\ \hline 
T500I1P100PL20TL50    & 1.122          & 1.380          & \textbf{1.844} &          1.183  & 1.714          &    1.176 \\ \hline 
T500I0.1P50PL10TL40   & \textbf{1.596} & \textbf{2.668} & \textbf{3.438} &  \textbf{5.135} & 6.088          &    6.595 \\ \hline 
T500I0.4P250PL10TL120 & \textbf{1.010} & \textbf{2.050} & \textbf{2.891} &  \textbf{4.186} & \textbf{5.021} &    \textbf{5.377}\\ \hline 
T500I0.1P100PL20TL50  & \textbf{1.229} & \textbf{2.155} & \textbf{2.875} &  \textbf{4.279} & \textbf{5.455} &    5.595 \\ \hline 
T500I0.4P150PL40TL80  & \textbf{1.142} & \textbf{2.102} & \textbf{2.709} &  \textbf{3.742} & 3.660          &    3.789 \\ \hline 
T500I0.1P250PL10TL40  & \textbf{1.176} & \textbf{2.179} & \textbf{3.003} &  \textbf{3.910} & \textbf{4.999} &    5.407 \\ \hline 
 Total average        & \textbf{1.270} & \textbf{2.142} & \textbf{2.867} &  \textbf{3.662} & 4.250          &    4.424 \\ \hline 
\end{tabular}


==> tables/avg_speedup_fimiseq.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40   &    1.395        &    1.884        &    2.111 &    \textbf{2.537} &    \textbf{3.549} &    \textbf{3.725} \\ \hline 
T500I0.1P50PL20TL40   &    1.492        &    2.536        &    3.371 &    4.554          &    \textbf{5.991} &    \textbf{6.957} \\ \hline 
T500I0.4P250PL20TL80  &    0.807        &    1.530        &    1.688 &    2.948          &    3.860          &    3.939          \\ \hline 
T500I1P100PL20TL50    &    \textbf{1.193}& \textbf{1.440} &    1.669 &    \textbf{1.784} &    \textbf{2.140} &    \textbf{2.357} \\ \hline 
T500I0.1P50PL10TL40   &    1.495        &    2.474        &    3.419 &    4.601          &    \textbf{6.331} &    \textbf{7.159} \\ \hline 
T500I0.4P250PL10TL120 &    0.828        &    1.474        &    2.032 &    3.174          &    4.350          &    5.090          \\ \hline 
T500I0.1P100PL20TL50  &    1.141        &    1.974        &    2.546 &    3.882          &    5.399          &    \textbf{6.209} \\ \hline 
T500I0.4P150PL40TL80  &    1.013        &    1.749        &    2.368 &    3.035          &    \textbf{4.113} &    \textbf{4.580} \\ \hline 
T500I0.1P250PL10TL40  &    1.056        &    1.878        &    2.427 &    3.546          &    4.891          &    \textbf{5.914} \\ \hline 
 Total average        &    1.158        &    1.882        &    2.403 &    3.340          &    \textbf{4.514} &    \textbf{5.103} \\ \hline 
\end{tabular}


==> tables/avg_speedup_reserv.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40    & \textbf{1.669} & \textbf{2.628} & \textbf{3.426} & \textbf{4.677} & \textbf{4.853} &    \textbf{6.223} \\ \hline 
T500I0.1P50PL20TL40    & 1.508          & \textbf{2.681} & \textbf{3.617} & 4.468          & 5.292          &    6.128          \\ \hline 
T500I0.4P250PL20TL80   & \textbf{1.637} & \textbf{2.644} & \textbf{4.135} & \textbf{6.191} & \textbf{6.530} &    \textbf{8.589} \\ \hline 
T500I1P100PL20TL50     & \textbf{1.221} & \textbf{1.650} & \textbf{2.199} & \textbf{3.010} & \textbf{3.984} &    \textbf{4.648} \\ \hline 
T500I0.1P50PL10TL40    & 1.523          & 2.633          & 3.380          & \textbf{5.342} & \textbf{7.058} &    \textbf{8.493} \\ \hline 
T500I0.4P250PL10TL120  & \textbf{1.389} & \textbf{2.481} & \textbf{3.470} & \textbf{4.932} & \textbf{6.249} &    \textbf{7.137} \\ \hline 
T500I0.1P100PL20TL50   & \textbf{1.289} & \textbf{2.212} & \textbf{2.946} & \textbf{4.811} & \textbf{6.431} &    \textbf{8.493} \\ \hline 
T500I0.4P150PL40TL80   & \textbf{1.322} & \textbf{2.336} & \textbf{3.106} & \textbf{4.290} & \textbf{5.043} &    \textbf{5.096} \\ \hline 
T500I0.1P250PL10TL40   & \textbf{1.314} & \textbf{2.321} & \textbf{3.064} & \textbf{5.009} & \textbf{6.938} &    \textbf{8.200} \\ \hline 
 Total average         & \textbf{1.430} & \textbf{2.399} & \textbf{3.260} & \textbf{4.748} & \textbf{5.804} &    \textbf{7.001} \\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-19869-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.349 &    1.918 &    2.423 &    3.037 &    3.532 &    3.578\\ \hline 
T500I0.1P50PL20TL40  &    1.417 &    2.399 &    3.040 &    4.280 &    6.113 &    6.761\\ \hline 
T500I0.4P250PL20TL80  &    0.771 &    1.471 &    1.906 &    2.928 &    4.108 &    4.703\\ \hline 
T500I1P100PL20TL50  &    1.020 &    1.520 &    1.824 &    1.939 &    2.281 &    2.273\\ \hline 
T500I0.1P50PL10TL40  &    1.345 &    2.264 &    3.103 &    4.538 &    6.386 &    7.385\\ \hline 
T500I0.4P250PL10TL120  &    0.759 &    1.471 &    2.101 &    3.044 &    4.159 &    4.985\\ \hline 
T500I0.1P100PL20TL50  &    1.062 &    1.832 &    2.413 &    3.660 &    5.349 &    6.110\\ \hline 
T500I0.4P150PL40TL80  &    0.965 &    1.635 &    2.282 &    3.163 &    4.121 &    4.658\\ \hline 
T500I0.1P250PL10TL40  &    0.985 &    1.724 &    2.285 &    3.513 &    4.830 &    5.778\\ \hline 
 Total average  &    1.075 &    1.804 &    2.375 &    3.345 &    4.542 &    5.137\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-19869-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.524 &    2.209 &    2.889 &    2.649 &    2.972 &    3.255\\ \hline 
T500I0.1P50PL20TL40  &    1.502 &    2.553 &    3.452 &    4.829 &    6.372 &    7.973\\ \hline 
T500I0.4P250PL20TL80  &    0.945 &    1.838 &    2.882 &    3.679 &    4.813 &    5.374\\ \hline 
T500I1P100PL20TL50  &    1.116 &    1.498 &    1.980 &    1.697 &    2.763 &    2.051\\ \hline 
T500I0.1P50PL10TL40  &    1.371 &    2.244 &    2.633 &    4.862 &    6.194 &    7.461\\ \hline 
T500I0.4P250PL10TL120  &    0.879 &    2.030 &    2.549 &    4.011 &    5.553 &    6.273\\ \hline 
T500I0.1P100PL20TL50  &    1.122 &    1.932 &    2.237 &    3.869 &    5.583 &    5.885\\ \hline 
T500I0.4P150PL40TL80  &    1.076 &    1.955 &    2.591 &    3.630 &    4.776 &    3.156\\ \hline 
T500I0.1P250PL10TL40  &    1.100 &    1.898 &    2.791 &    3.954 &    5.525 &    6.239\\ \hline 
 Total average  &    1.182 &    2.018 &    2.667 &    3.687 &    4.950 &    5.296\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-19869-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.628 &    2.347 &    3.372 &    4.776 &    6.202 &    6.893\\ \hline 
T500I0.1P50PL20TL40  &    1.455 &    2.550 &    3.093 &    4.076 &    5.670 &    6.342\\ \hline 
T500I0.4P250PL20TL80  &    1.453 &    2.757 &    3.965 &    5.761 &    6.208 &    8.430\\ \hline 
T500I1P100PL20TL50  &    1.121 &    1.923 &    2.374 &    2.841 &    4.026 &    5.753\\ \hline 
T500I0.1P50PL10TL40  &    1.380 &    2.521 &    3.281 &    4.464 &    6.772 &    8.860\\ \hline 
T500I0.4P250PL10TL120  &    1.216 &    2.249 &    3.117 &    4.584 &    6.179 &    7.067\\ \hline 
T500I0.1P100PL20TL50  &    1.172 &    2.071 &    2.767 &    3.802 &    6.840 &    8.967\\ \hline 
T500I0.4P150PL40TL80  &    1.211 &    2.155 &    2.858 &    3.789 &    4.976 &    5.423\\ \hline 
T500I0.1P250PL10TL40  &    1.243 &    2.161 &    2.930 &    4.606 &    6.863 &    7.793\\ \hline 
 Total average  &    1.320 &    2.304 &    3.084 &    4.300 &    5.971 &    7.281\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-26492-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.350 &    2.028 &    2.446 &    2.978 &    3.686 &    3.583\\ \hline 
T500I0.1P50PL20TL40  &    1.415 &    2.388 &    3.301 &    4.523 &    5.895 &    6.811\\ \hline 
T500I0.4P250PL20TL80  &    0.781 &    1.372 &    1.960 &    2.953 &    3.914 &    3.855\\ \hline 
T500I1P100PL20TL50  &    1.052 &    1.511 &    1.602 &    2.119 &    2.228 &    2.165\\ \hline 
T500I0.1P50PL10TL40  &    1.312 &    2.287 &    3.112 &    4.364 &    6.190 &    7.308\\ \hline 
T500I0.4P250PL10TL120  &    0.712 &    1.353 &    2.089 &    3.103 &    4.172 &    5.170\\ \hline 
T500I0.1P100PL20TL50  &    1.078 &    1.845 &    2.672 &    3.589 &    5.354 &    6.220\\ \hline 
T500I0.4P150PL40TL80  &    0.893 &    1.658 &    2.252 &    3.135 &    4.205 &    4.555\\ \hline 
T500I0.1P250PL10TL40  &    0.969 &    1.765 &    2.325 &    3.387 &    5.213 &    5.999\\ \hline 
 Total average  &    1.062 &    1.801 &    2.418 &    3.350 &    4.540 &    5.074\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-26492-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.504 &    2.100 &    2.874 &    2.584 &    2.969 &    3.197\\ \hline 
T500I0.1P50PL20TL40  &    1.456 &    2.605 &    3.469 &    5.105 &    6.153 &    6.739\\ \hline 
T500I0.4P250PL20TL80  &    0.950 &    1.985 &    2.528 &    3.966 &    5.153 &    5.580\\ \hline 
T500I1P100PL20TL50  &    0.969 &    1.662 &    1.913 &    1.507 &    2.190 &    2.012\\ \hline 
T500I0.1P50PL10TL40  &    1.305 &    2.613 &    3.485 &    4.846 &    5.478 &    7.338\\ \hline 
T500I0.4P250PL10TL120  &    0.860 &    1.927 &    2.624 &    3.943 &    5.491 &    5.783\\ \hline 
T500I0.1P100PL20TL50  &    1.125 &    2.041 &    2.724 &    3.723 &    5.490 &    6.278\\ \hline 
T500I0.4P150PL40TL80  &    1.079 &    1.986 &    2.645 &    3.774 &    4.761 &    5.045\\ \hline 
T500I0.1P250PL10TL40  &    1.090 &    2.020 &    2.740 &    3.926 &    5.100 &    6.577\\ \hline 
 Total average  &    1.149 &    2.104 &    2.778 &    3.708 &    4.754 &    5.395\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-26492-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.551 &    2.463 &    3.107 &    4.546 &    5.588 &    5.466\\ \hline 
T500I0.1P50PL20TL40  &    1.405 &    2.235 &    3.127 &    3.674 &    5.568 &    6.561\\ \hline 
T500I0.4P250PL20TL80  &    1.525 &    2.755 &    3.695 &    5.460 &    6.556 &    8.632\\ \hline 
T500I1P100PL20TL50  &    1.207 &    1.713 &    2.429 &    2.627 &    3.756 &    4.702\\ \hline 
T500I0.1P50PL10TL40  &    1.413 &    2.377 &    2.759 &    4.557 &    7.476 &    8.220\\ \hline 
T500I0.4P250PL10TL120  &    1.232 &    2.306 &    2.978 &    4.725 &    6.363 &    7.016\\ \hline 
T500I0.1P100PL20TL50  &    1.167 &    2.074 &    2.700 &    3.955 &    7.386 &    8.905\\ \hline 
T500I0.4P150PL40TL80  &    1.184 &    2.147 &    1.569 &    3.897 &    4.760 &    5.201\\ \hline 
T500I0.1P250PL10TL40  &    1.220 &    2.111 &    2.492 &    4.293 &    7.112 &    8.342\\ \hline 
 Total average  &    1.323 &    2.242 &    2.762 &    4.193 &    6.063 &    7.005\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-33115-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.296 &    1.904 &    2.541 &    2.931 &    3.546 &    3.701\\ \hline 
T500I0.1P50PL20TL40  &    1.339 &    2.354 &    3.164 &    4.520 &    5.903 &    6.697\\ \hline 
T500I0.4P250PL20TL80  &    0.788 &    1.402 &    1.946 &    2.528 &    3.779 &    4.643\\ \hline 
T500I1P100PL20TL50  &    1.090 &    1.459 &    1.757 &    1.934 &    2.041 &    2.384\\ \hline 
T500I0.1P50PL10TL40  &    1.390 &    2.262 &    3.191 &    4.472 &    6.263 &    6.981\\ \hline 
T500I0.4P250PL10TL120  &    0.790 &    1.287 &    2.070 &    3.162 &    4.289 &    5.027\\ \hline 
T500I0.1P100PL20TL50  &    1.079 &    1.855 &    2.482 &    3.628 &    5.407 &    6.258\\ \hline 
T500I0.4P150PL40TL80  &    0.989 &    1.687 &    2.340 &    3.069 &    4.052 &    4.313\\ \hline 
T500I0.1P250PL10TL40  &    0.980 &    1.719 &    2.340 &    3.415 &    5.035 &    5.770\\ \hline 
 Total average  &    1.082 &    1.770 &    2.426 &    3.295 &    4.480 &    5.086\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-33115-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.436 &    2.189 &    3.113 &    2.644 &    2.997 &    3.335\\ \hline 
T500I0.1P50PL20TL40  &    1.422 &    2.603 &    2.546 &    5.020 &    6.261 &    7.438\\ \hline 
T500I0.4P250PL20TL80  &    0.986 &    1.889 &    2.891 &    4.091 &    4.720 &    4.922\\ \hline 
T500I1P100PL20TL50  &    1.086 &    1.562 &    1.302 &    1.564 &    2.396 &    1.693\\ \hline 
T500I0.1P50PL10TL40  &    1.366 &    2.483 &    3.383 &    4.992 &    5.939 &    7.696\\ \hline 
T500I0.4P250PL10TL120  &    0.857 &    1.892 &    2.760 &    4.042 &    5.420 &    6.282\\ \hline 
T500I0.1P100PL20TL50  &    1.122 &    1.953 &    2.637 &    3.782 &    5.600 &    6.421\\ \hline 
T500I0.4P150PL40TL80  &    1.087 &    1.980 &    2.663 &    3.576 &    4.793 &    5.132\\ \hline 
T500I0.1P250PL10TL40  &    1.021 &    2.061 &    2.775 &    3.806 &    5.898 &    6.064\\ \hline 
 Total average  &    1.154 &    2.068 &    2.674 &    3.724 &    4.892 &    5.443\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-10000-33115-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.662 &    2.227 &    3.100 &    3.362 &    5.583 &    6.690\\ \hline 
T500I0.1P50PL20TL40  &    1.426 &    2.478 &    2.782 &    4.578 &    4.885 &    6.674\\ \hline 
T500I0.4P250PL20TL80  &    1.491 &    2.635 &    3.745 &    5.280 &    7.219 &    8.103\\ \hline 
T500I1P100PL20TL50  &    1.188 &    1.706 &    2.347 &    2.792 &    3.632 &    5.037\\ \hline 
T500I0.1P50PL10TL40  &    1.429 &    2.452 &    2.907 &    4.964 &    7.401 &    8.508\\ \hline 
T500I0.4P250PL10TL120  &    1.240 &    2.285 &    2.999 &    4.556 &    6.181 &    7.108\\ \hline 
T500I0.1P100PL20TL50  &    1.158 &    2.076 &    2.787 &    3.764 &    7.085 &    8.843\\ \hline 
T500I0.4P150PL40TL80  &    1.201 &    2.021 &    2.852 &    3.952 &    4.970 &    5.501\\ \hline 
T500I0.1P250PL10TL40  &    1.235 &    2.199 &    2.923 &    4.736 &    7.157 &    8.508\\ \hline 
 Total average  &    1.337 &    2.231 &    2.938 &    4.221 &    6.013 &    7.219\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-13246-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.345 &    2.047 &    2.315 &    2.680 &    3.493 &    3.590\\ \hline 
T500I0.1P50PL20TL40  &    1.391 &    2.430 &    3.236 &    3.778 &    5.983 &    6.931\\ \hline 
T500I0.4P250PL20TL80  &    0.778 &    1.431 &    2.004 &    2.940 &    3.750 &    4.362\\ \hline 
T500I1P100PL20TL50  &    1.131 &    1.531 &    1.734 &    1.880 &    2.001 &    2.287\\ \hline 
T500I0.1P50PL10TL40  &    1.350 &    2.327 &    3.128 &    4.398 &    6.417 &    7.121\\ \hline 
T500I0.4P250PL10TL120  &    0.797 &    1.432 &    2.084 &    2.914 &    4.096 &    5.065\\ \hline 
T500I0.1P100PL20TL50  &    1.066 &    1.785 &    2.561 &    3.773 &    5.359 &    6.247\\ \hline 
T500I0.4P150PL40TL80  &    0.969 &    1.704 &    2.280 &    3.155 &    4.059 &    4.391\\ \hline 
T500I0.1P250PL10TL40  &    1.025 &    1.842 &    2.346 &    3.516 &    4.739 &    5.629\\ \hline 
 Total average  &    1.095 &    1.836 &    2.410 &    3.226 &    4.433 &    5.069\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-13246-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.512 &    2.358 &    2.718 &    2.711 &    2.873 &    3.170\\ \hline 
T500I0.1P50PL20TL40  &    1.430 &    2.715 &    3.416 &    5.149 &    6.644 &    6.130\\ \hline 
T500I0.4P250PL20TL80  &    0.949 &    1.794 &    2.903 &    3.602 &    4.729 &    5.293\\ \hline 
T500I1P100PL20TL50  &    1.026 &    1.144 &    2.015 &    1.731 &    2.362 &    2.017\\ \hline 
T500I0.1P50PL10TL40  &    1.340 &    2.451 &    3.463 &    4.981 &    6.204 &    7.237\\ \hline 
T500I0.4P250PL10TL120  &    0.911 &    1.894 &    2.672 &    3.939 &    5.196 &    5.896\\ \hline 
T500I0.1P100PL20TL50  &    1.099 &    1.965 &    2.737 &    3.765 &    4.698 &    5.872\\ \hline 
T500I0.4P150PL40TL80  &    1.055 &    2.013 &    2.600 &    3.665 &    4.456 &    3.495\\ \hline 
T500I0.1P250PL10TL40  &    1.087 &    1.900 &    2.730 &    3.956 &    5.044 &    6.895\\ \hline 
 Total average  &    1.157 &    2.026 &    2.806 &    3.722 &    4.690 &    5.112\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-13246-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.523 &    2.358 &    3.184 &    4.582 &    5.544 &    6.730\\ \hline 
T500I0.1P50PL20TL40  &    1.451 &    2.571 &    2.869 &    4.228 &    5.341 &    5.930\\ \hline 
T500I0.4P250PL20TL80  &    1.502 &    2.715 &    3.564 &    5.009 &    6.656 &    7.965\\ \hline 
T500I1P100PL20TL50  &    1.195 &    1.881 &    2.227 &    2.845 &    3.779 &    3.848\\ \hline 
T500I0.1P50PL10TL40  &    1.341 &    2.466 &    3.187 &    4.322 &    7.177 &    8.273\\ \hline 
T500I0.4P250PL10TL120  &    1.218 &    2.230 &    3.068 &    4.660 &    6.234 &    6.955\\ \hline 
T500I0.1P100PL20TL50  &    1.175 &    1.987 &    2.589 &    4.181 &    6.752 &    8.382\\ \hline 
T500I0.4P150PL40TL80  &    1.201 &    2.065 &    2.769 &    3.855 &    4.732 &    5.341\\ \hline 
T500I0.1P250PL10TL40  &    1.204 &    2.189 &    2.860 &    4.685 &    6.393 &    8.155\\ \hline 
 Total average  &    1.312 &    2.274 &    2.924 &    4.263 &    5.845 &    6.842\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-19869-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.375 &    1.877 &    2.424 &    3.003 &    3.377 &    3.746\\ \hline 
T500I0.1P50PL20TL40  &    1.355 &    2.454 &    3.307 &    4.515 &    5.888 &    6.738\\ \hline 
T500I0.4P250PL20TL80  &    0.781 &    1.405 &    1.807 &    2.848 &    4.041 &    4.494\\ \hline 
T500I1P100PL20TL50  &    1.025 &    1.472 &    1.624 &    1.742 &    2.183 &    2.216\\ \hline 
T500I0.1P50PL10TL40  &    1.399 &    2.284 &    3.115 &    4.367 &    6.258 &    6.912\\ \hline 
T500I0.4P250PL10TL120  &    0.791 &    1.464 &    1.920 &    2.855 &    4.070 &    5.085\\ \hline 
T500I0.1P100PL20TL50  &    1.058 &    1.858 &    2.443 &    3.579 &    5.311 &    6.104\\ \hline 
T500I0.4P150PL40TL80  &    0.945 &    1.699 &    2.178 &    2.581 &    3.915 &    4.480\\ \hline 
T500I0.1P250PL10TL40  &    0.969 &    1.623 &    2.295 &    3.445 &    4.848 &    5.931\\ \hline 
 Total average  &    1.078 &    1.793 &    2.346 &    3.215 &    4.432 &    5.078\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-19869-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.488 &    2.126 &    2.804 &    2.660 &    2.720 &    3.186\\ \hline 
T500I0.1P50PL20TL40  &    1.490 &    2.584 &    3.438 &    5.201 &    5.542 &    6.274\\ \hline 
T500I0.4P250PL20TL80  &    0.959 &    1.857 &    2.712 &    4.042 &    5.248 &    5.628\\ \hline 
T500I1P100PL20TL50  &    1.117 &    1.576 &    1.805 &    1.643 &    2.398 &    1.978\\ \hline 
T500I0.1P50PL10TL40  &    1.286 &    2.354 &    3.382 &    5.016 &    5.869 &    7.517\\ \hline 
T500I0.4P250PL10TL120  &    0.848 &    1.897 &    2.620 &    3.883 &    5.451 &    6.101\\ \hline 
T500I0.1P100PL20TL50  &    1.119 &    1.979 &    2.825 &    3.854 &    4.928 &    6.737\\ \hline 
T500I0.4P150PL40TL80  &    1.082 &    2.008 &    2.267 &    3.616 &    4.630 &    5.152\\ \hline 
T500I0.1P250PL10TL40  &    1.073 &    2.110 &    2.734 &    4.105 &    5.232 &    6.089\\ \hline 
 Total average  &    1.163 &    2.055 &    2.732 &    3.780 &    4.669 &    5.407\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-19869-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.575 &    2.472 &    3.123 &    4.695 &    4.878 &    6.525\\ \hline 
T500I0.1P50PL20TL40  &    1.380 &    2.340 &    2.925 &    4.095 &    4.786 &    6.015\\ \hline 
T500I0.4P250PL20TL80  &    1.482 &    2.803 &    3.770 &    5.525 &    6.059 &    8.403\\ \hline 
T500I1P100PL20TL50  &    1.195 &    1.900 &    2.340 &    2.741 &    4.367 &    4.374\\ \hline 
T500I0.1P50PL10TL40  &    1.429 &    2.380 &    2.729 &    4.566 &    6.926 &    8.419\\ \hline 
T500I0.4P250PL10TL120  &    1.228 &    2.271 &    2.996 &    4.483 &    6.040 &    6.983\\ \hline 
T500I0.1P100PL20TL50  &    1.158 &    1.965 &    2.596 &    3.644 &    6.791 &    7.951\\ \hline 
T500I0.4P150PL40TL80  &    1.163 &    2.169 &    2.809 &    3.870 &    4.803 &    5.031\\ \hline 
T500I0.1P250PL10TL40  &    1.228 &    2.126 &    2.884 &    4.848 &    6.956 &    8.288\\ \hline 
 Total average  &    1.315 &    2.270 &    2.908 &    4.274 &    5.734 &    6.888\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-26492-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.354 &    1.817 &    1.881 &    2.754 &    2.573 &    3.474\\ \hline 
T500I0.1P50PL20TL40  &    1.313 &    2.455 &    3.253 &    4.533 &    4.807 &    6.695\\ \hline 
T500I0.4P250PL20TL80  &    0.744 &    1.445 &    1.935 &    2.503 &    3.764 &    4.532\\ \hline 
T500I1P100PL20TL50  &    1.100 &    1.625 &    1.695 &    1.896 &    2.153 &    2.270\\ \hline 
T500I0.1P50PL10TL40  &    1.413 &    2.350 &    3.243 &    4.549 &    6.127 &    7.109\\ \hline 
T500I0.4P250PL10TL120  &    0.783 &    1.418 &    1.962 &    2.960 &    4.379 &    4.917\\ \hline 
T500I0.1P100PL20TL50  &    1.030 &    1.773 &    2.410 &    3.662 &    5.397 &    6.176\\ \hline 
T500I0.4P150PL40TL80  &    0.964 &    1.693 &    2.272 &    3.128 &    3.957 &    4.327\\ \hline 
T500I0.1P250PL10TL40  &    1.008 &    1.633 &    2.413 &    3.478 &    4.914 &    5.653\\ \hline 
 Total average  &    1.079 &    1.801 &    2.340 &    3.274 &    4.230 &    5.017\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-26492-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.407 &    2.014 &    2.760 &    2.850 &    2.246 &    3.501\\ \hline 
T500I0.1P50PL20TL40  &    1.469 &    1.978 &    3.600 &    5.185 &    5.718 &    6.319\\ \hline 
T500I0.4P250PL20TL80  &    0.987 &    2.025 &    3.130 &    3.630 &    4.386 &    5.519\\ \hline 
T500I1P100PL20TL50  &    0.991 &    1.641 &    1.799 &    1.616 &    2.685 &    2.031\\ \hline 
T500I0.1P50PL10TL40  &    1.259 &    2.432 &    3.346 &    4.838 &    5.742 &    7.503\\ \hline 
T500I0.4P250PL10TL120  &    0.949 &    1.955 &    2.648 &    3.906 &    5.402 &    6.147\\ \hline 
T500I0.1P100PL20TL50  &    1.101 &    1.892 &    2.426 &    3.694 &    5.510 &    6.348\\ \hline 
T500I0.4P150PL40TL80  &    1.069 &    2.020 &    1.408 &    3.692 &    4.580 &    4.954\\ \hline 
T500I0.1P250PL10TL40  &    1.080 &    1.916 &    2.413 &    4.096 &    5.412 &    6.085\\ \hline 
 Total average  &    1.146 &    1.986 &    2.615 &    3.723 &    4.631 &    5.379\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-26492-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.543 &    2.510 &    3.219 &    3.264 &    4.625 &    6.006\\ \hline 
T500I0.1P50PL20TL40  &    1.398 &    2.514 &    3.211 &    3.904 &    4.670 &    5.486\\ \hline 
T500I0.4P250PL20TL80  &    1.403 &    2.665 &    3.810 &    5.079 &    6.741 &    8.457\\ \hline 
T500I1P100PL20TL50  &    1.207 &    1.588 &    1.969 &    2.760 &    3.240 &    4.466\\ \hline 
T500I0.1P50PL10TL40  &    1.397 &    2.382 &    3.104 &    4.453 &    6.714 &    8.209\\ \hline 
T500I0.4P250PL10TL120  &    1.218 &    2.162 &    3.001 &    4.557 &    6.084 &    7.103\\ \hline 
T500I0.1P100PL20TL50  &    1.167 &    1.999 &    2.614 &    3.787 &    6.646 &    8.001\\ \hline 
T500I0.4P150PL40TL80  &    1.203 &    2.065 &    2.834 &    3.805 &    4.729 &    5.132\\ \hline 
T500I0.1P250PL10TL40  &    1.224 &    2.131 &    2.788 &    4.443 &    6.142 &    8.334\\ \hline 
 Total average  &    1.307 &    2.224 &    2.950 &    4.006 &    5.510 &    6.799\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-33115-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.236 &    1.934 &    2.325 &    2.778 &    3.513 &    3.330\\ \hline 
T500I0.1P50PL20TL40  &    1.315 &    2.414 &    3.200 &    4.454 &    6.058 &    6.459\\ \hline 
T500I0.4P250PL20TL80  &    0.787 &    1.503 &    1.985 &    2.910 &    4.046 &    4.757\\ \hline 
T500I1P100PL20TL50  &    1.084 &    1.452 &    1.779 &    1.934 &    2.177 &    1.924\\ \hline 
T500I0.1P50PL10TL40  &    1.356 &    2.384 &    3.068 &    4.532 &    6.329 &    7.184\\ \hline 
T500I0.4P250PL10TL120  &    0.779 &    1.494 &    1.945 &    2.967 &    4.128 &    4.979\\ \hline 
T500I0.1P100PL20TL50  &    1.086 &    1.842 &    2.377 &    3.678 &    5.386 &    5.873\\ \hline 
T500I0.4P150PL40TL80  &    0.938 &    1.655 &    2.170 &    3.027 &    3.986 &    4.480\\ \hline 
T500I0.1P250PL10TL40  &    0.999 &    1.683 &    2.284 &    3.425 &    5.015 &    5.946\\ \hline 
 Total average  &    1.064 &    1.818 &    2.348 &    3.300 &    4.515 &    4.993\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-33115-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.433 &    2.200 &    3.031 &    2.676 &    3.084 &    3.152\\ \hline 
T500I0.1P50PL20TL40  &    1.447 &    2.550 &    3.017 &    4.936 &    5.700 &    7.993\\ \hline 
T500I0.4P250PL20TL80  &    0.973 &    2.038 &    2.995 &    3.603 &    4.586 &    5.222\\ \hline 
T500I1P100PL20TL50  &    1.127 &    1.431 &    1.920 &    1.575 &    2.227 &    2.009\\ \hline 
T500I0.1P50PL10TL40  &    1.391 &    2.360 &    3.069 &    5.107 &    6.054 &    6.917\\ \hline 
T500I0.4P250PL10TL120  &    0.936 &    1.963 &    2.596 &    3.933 &    5.425 &    6.211\\ \hline 
T500I0.1P100PL20TL50  &    1.068 &    1.944 &    2.596 &    3.744 &    5.041 &    5.899\\ \hline 
T500I0.4P150PL40TL80  &    1.063 &    1.973 &    2.526 &    3.562 &    4.734 &    4.924\\ \hline 
T500I0.1P250PL10TL40  &    1.074 &    2.047 &    2.685 &    4.037 &    5.339 &    6.543\\ \hline 
 Total average  &    1.168 &    2.056 &    2.715 &    3.686 &    4.688 &    5.430\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-33115-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.557 &    2.376 &    2.825 &    4.181 &    4.919 &    5.290\\ \hline 
T500I0.1P50PL20TL40  &    1.359 &    2.487 &    2.954 &    4.224 &    5.190 &    5.364\\ \hline 
T500I0.4P250PL20TL80  &    1.484 &    2.772 &    3.782 &    5.120 &    6.231 &    8.514\\ \hline 
T500I1P100PL20TL50  &    1.201 &    1.664 &    2.170 &    2.456 &    3.966 &    4.878\\ \hline 
T500I0.1P50PL10TL40  &    1.421 &    2.423 &    3.074 &    4.549 &    6.927 &    8.365\\ \hline 
T500I0.4P250PL10TL120  &    1.238 &    2.264 &    3.062 &    4.607 &    6.129 &    7.075\\ \hline 
T500I0.1P100PL20TL50  &    1.175 &    1.998 &    2.530 &    4.040 &    6.156 &    8.572\\ \hline 
T500I0.4P150PL40TL80  &    1.191 &    2.067 &    2.720 &    3.756 &    4.952 &    5.139\\ \hline 
T500I0.1P250PL10TL40  &    1.199 &    2.179 &    2.676 &    3.860 &    6.896 &    8.114\\ \hline 
 Total average  &    1.314 &    2.248 &    2.866 &    4.088 &    5.707 &    6.812\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-39738-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.389 &    1.877 &    2.457 &    2.883 &    3.268 &    3.681\\ \hline 
T500I0.1P50PL20TL40  &    1.388 &    2.417 &    3.211 &    4.453 &    5.939 &    6.709\\ \hline 
T500I0.4P250PL20TL80  &    0.777 &    1.477 &    1.868 &    2.562 &    3.993 &    4.497\\ \hline 
T500I1P100PL20TL50  &    1.087 &    1.529 &    1.785 &    2.028 &    2.224 &    2.283\\ \hline 
T500I0.1P50PL10TL40  &    1.367 &    2.304 &    3.147 &    4.280 &    6.253 &    7.184\\ \hline 
T500I0.4P250PL10TL120  &    0.749 &    1.467 &    1.950 &    2.611 &    4.020 &    4.997\\ \hline 
T500I0.1P100PL20TL50  &    1.077 &    1.881 &    2.495 &    3.521 &    5.156 &    6.283\\ \hline 
T500I0.4P150PL40TL80  &    0.929 &    1.672 &    2.211 &    2.196 &    3.892 &    4.546\\ \hline 
T500I0.1P250PL10TL40  &    0.996 &    1.763 &    2.258 &    3.389 &    5.011 &    5.851\\ \hline 
 Total average  &    1.084 &    1.821 &    2.376 &    3.103 &    4.417 &    5.115\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-39738-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.433 &    2.244 &    3.097 &    2.868 &    2.880 &    3.399\\ \hline 
T500I0.1P50PL20TL40  &    1.407 &    2.510 &    3.450 &    4.849 &    5.785 &    7.211\\ \hline 
T500I0.4P250PL20TL80  &    0.914 &    1.951 &    2.921 &    3.960 &    4.808 &    5.347\\ \hline 
T500I1P100PL20TL50  &    1.094 &    1.679 &    1.920 &    1.700 &    2.348 &    1.975\\ \hline 
T500I0.1P50PL10TL40  &    1.396 &    2.492 &    3.208 &    4.930 &    5.920 &    7.487\\ \hline 
T500I0.4P250PL10TL120  &    0.943 &    1.993 &    2.703 &    4.212 &    5.455 &    5.671\\ \hline 
T500I0.1P100PL20TL50  &    1.120 &    1.974 &    2.687 &    4.198 &    5.320 &    6.394\\ \hline 
T500I0.4P150PL40TL80  &    1.059 &    2.005 &    2.660 &    3.539 &    4.326 &    4.960\\ \hline 
T500I0.1P250PL10TL40  &    1.112 &    1.838 &    2.729 &    4.276 &    5.629 &    6.186\\ \hline 
 Total average  &    1.164 &    2.076 &    2.820 &    3.837 &    4.719 &    5.403\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-14450-39738-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.570 &    2.497 &    2.998 &    4.003 &    5.733 &    6.238\\ \hline 
T500I0.1P50PL20TL40  &    1.399 &    2.478 &    2.488 &    4.478 &    5.074 &    5.954\\ \hline 
T500I0.4P250PL20TL80  &    1.474 &    2.652 &    3.548 &    5.381 &    6.187 &    8.493\\ \hline 
T500I1P100PL20TL50  &    1.226 &    1.788 &    2.113 &    2.597 &    3.536 &    4.414\\ \hline 
T500I0.1P50PL10TL40  &    1.393 &    2.415 &    3.095 &    4.109 &    7.039 &    8.142\\ \hline 
T500I0.4P250PL10TL120  &    1.223 &    2.297 &    3.035 &    4.548 &    6.077 &    6.995\\ \hline 
T500I0.1P100PL20TL50  &    1.144 &    1.969 &    2.645 &    4.218 &    6.588 &    8.010\\ \hline 
T500I0.4P150PL40TL80  &    1.189 &    2.019 &    2.807 &    3.667 &    4.883 &    5.292\\ \hline 
T500I0.1P250PL10TL40  &    1.220 &    2.155 &    2.781 &    4.229 &    7.065 &    8.137\\ \hline 
 Total average  &    1.315 &    2.252 &    2.834 &    4.137 &    5.798 &    6.853\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-19869-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.348 &    2.115 &    2.571 &    2.970 &    3.542 &    3.453\\ \hline 
T500I0.1P50PL20TL40  &    1.409 &    2.395 &    2.996 &    4.579 &    6.050 &    6.612\\ \hline 
T500I0.4P250PL20TL80  &    0.757 &    1.372 &    2.042 &    2.737 &    3.921 &    4.712\\ \hline 
T500I1P100PL20TL50  &    1.171 &    1.546 &    1.581 &    1.968 &    2.159 &    2.297\\ \hline 
T500I0.1P50PL10TL40  &    1.354 &    2.351 &    3.143 &    4.447 &    6.313 &    7.193\\ \hline 
T500I0.4P250PL10TL120  &    0.757 &    1.362 &    1.959 &    3.092 &    4.259 &    5.012\\ \hline 
T500I0.1P100PL20TL50  &    1.049 &    1.872 &    2.314 &    3.704 &    5.278 &    6.321\\ \hline 
T500I0.4P150PL40TL80  &    0.965 &    1.633 &    2.206 &    3.041 &    4.078 &    4.533\\ \hline 
T500I0.1P250PL10TL40  &    0.958 &    1.743 &    2.332 &    3.495 &    5.118 &    5.674\\ \hline 
 Total average  &    1.085 &    1.821 &    2.349 &    3.337 &    4.524 &    5.090\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-19869-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.467 &    2.244 &    3.151 &    2.930 &    2.720 &    3.182\\ \hline 
T500I0.1P50PL20TL40  &    1.474 &    2.461 &    3.226 &    5.050 &    6.198 &    7.335\\ \hline 
T500I0.4P250PL20TL80  &    0.969 &    1.820 &    2.992 &    3.345 &    4.360 &    5.501\\ \hline 
T500I1P100PL20TL50  &    1.043 &    1.609 &    1.899 &    1.614 &    2.644 &    1.847\\ \hline 
T500I0.1P50PL10TL40  &    1.392 &    2.519 &    3.335 &    5.038 &    5.853 &    7.333\\ \hline 
T500I0.4P250PL10TL120  &    0.944 &    1.915 &    2.780 &    3.822 &    5.649 &    6.162\\ \hline 
T500I0.1P100PL20TL50  &    1.116 &    2.057 &    2.653 &    3.867 &    5.438 &    6.039\\ \hline 
T500I0.4P150PL40TL80  &    1.058 &    1.985 &    2.652 &    3.379 &    4.455 &    4.742\\ \hline 
T500I0.1P250PL10TL40  &    1.077 &    1.992 &    2.612 &    3.840 &    5.288 &    5.750\\ \hline 
 Total average  &    1.171 &    2.067 &    2.811 &    3.654 &    4.734 &    5.321\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-19869-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.566 &    2.396 &    3.182 &    4.254 &    4.867 &    5.211\\ \hline 
T500I0.1P50PL20TL40  &    1.354 &    2.303 &    3.261 &    3.946 &    4.987 &    6.029\\ \hline 
T500I0.4P250PL20TL80  &    1.493 &    2.628 &    3.761 &    4.900 &    6.112 &    7.940\\ \hline 
T500I1P100PL20TL50  &    1.180 &    1.745 &    2.361 &    2.826 &    3.870 &    3.701\\ \hline 
T500I0.1P50PL10TL40  &    1.387 &    2.505 &    3.184 &    4.514 &    6.259 &    8.128\\ \hline 
T500I0.4P250PL10TL120  &    1.217 &    2.199 &    2.959 &    4.309 &    6.049 &    6.718\\ \hline 
T500I0.1P100PL20TL50  &    1.163 &    2.067 &    2.590 &    4.052 &    6.846 &    8.401\\ \hline 
T500I0.4P150PL40TL80  &    1.173 &    1.939 &    2.734 &    3.826 &    4.604 &    5.096\\ \hline 
T500I0.1P250PL10TL40  &    1.209 &    2.137 &    2.849 &    4.906 &    6.857 &    7.984\\ \hline 
 Total average  &    1.305 &    2.213 &    2.987 &    4.170 &    5.606 &    6.579\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-26492-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.220 &    2.110 &    2.269 &    3.017 &    3.073 &    3.714\\ \hline 
T500I0.1P50PL20TL40  &    1.353 &    2.412 &    3.302 &    4.609 &    5.839 &    6.583\\ \hline 
T500I0.4P250PL20TL80  &    0.784 &    1.407 &    1.970 &    2.687 &    3.766 &    4.826\\ \hline 
T500I1P100PL20TL50  &    1.152 &    1.502 &    1.670 &    1.952 &    2.163 &    2.160\\ \hline 
T500I0.1P50PL10TL40  &    1.373 &    2.264 &    3.081 &    4.682 &    6.259 &    7.066\\ \hline 
T500I0.4P250PL10TL120  &    0.785 &    1.429 &    1.986 &    3.052 &    4.092 &    5.001\\ \hline 
T500I0.1P100PL20TL50  &    1.075 &    1.771 &    2.474 &    3.632 &    5.297 &    6.340\\ \hline 
T500I0.4P150PL40TL80  &    0.978 &    1.584 &    2.274 &    3.131 &    4.061 &    4.413\\ \hline 
T500I0.1P250PL10TL40  &    1.000 &    1.722 &    2.361 &    3.354 &    4.846 &    5.783\\ \hline 
 Total average  &    1.080 &    1.800 &    2.376 &    3.346 &    4.377 &    5.098\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-26492-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.421 &    2.254 &    3.252 &    2.832 &    3.047 &    3.055\\ \hline 
T500I0.1P50PL20TL40  &    1.428 &    2.555 &    3.434 &    4.997 &    6.425 &    7.296\\ \hline 
T500I0.4P250PL20TL80  &    0.936 &    1.927 &    2.928 &    3.677 &    4.970 &    5.156\\ \hline 
T500I1P100PL20TL50  &    1.037 &    1.575 &    2.041 &    1.573 &    2.413 &    1.893\\ \hline 
T500I0.1P50PL10TL40  &    1.436 &    2.313 &    3.352 &    4.950 &    6.082 &    7.778\\ \hline 
T500I0.4P250PL10TL120  &    0.919 &    1.884 &    2.641 &    3.547 &    5.214 &    6.040\\ \hline 
T500I0.1P100PL20TL50  &    1.109 &    1.996 &    2.630 &    3.726 &    5.142 &    5.993\\ \hline 
T500I0.4P150PL40TL80  &    1.077 &    1.908 &    2.521 &    3.454 &    4.473 &    4.767\\ \hline 
T500I0.1P250PL10TL40  &    1.004 &    1.933 &    2.635 &    4.071 &    5.201 &    6.659\\ \hline 
 Total average  &    1.152 &    2.038 &    2.826 &    3.647 &    4.774 &    5.404\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-26492-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.546 &    2.347 &    3.060 &    4.299 &    5.165 &    5.331\\ \hline 
T500I0.1P50PL20TL40  &    1.290 &    2.380 &    2.948 &    4.238 &    5.704 &    6.591\\ \hline 
T500I0.4P250PL20TL80  &    1.434 &    2.649 &    3.615 &    5.243 &    5.917 &    7.824\\ \hline 
T500I1P100PL20TL50  &    1.122 &    1.828 &    2.044 &    2.475 &    3.216 &    4.309\\ \hline 
T500I0.1P50PL10TL40  &    1.419 &    2.345 &    2.905 &    4.345 &    6.761 &    8.257\\ \hline 
T500I0.4P250PL10TL120  &    1.212 &    2.197 &    2.971 &    4.376 &    6.064 &    6.611\\ \hline 
T500I0.1P100PL20TL50  &    1.154 &    1.982 &    2.493 &    3.636 &    7.013 &    7.989\\ \hline 
T500I0.4P150PL40TL80  &    1.168 &    2.110 &    2.650 &    3.765 &    4.780 &    5.314\\ \hline 
T500I0.1P250PL10TL40  &    1.199 &    2.030 &    2.794 &    4.484 &    6.686 &    7.955\\ \hline 
 Total average  &    1.283 &    2.208 &    2.831 &    4.096 &    5.701 &    6.687\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-33115-fpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimiseq{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.356 &    1.893 &    2.665 &    2.955 &    3.526 &    3.887\\ \hline 
T500I0.1P50PL20TL40  &    1.415 &    2.464 &    3.363 &    4.488 &    5.484 &    6.851\\ \hline 
T500I0.4P250PL20TL80  &    0.795 &    1.444 &    1.803 &    2.709 &    3.564 &    4.650\\ \hline 
T500I1P100PL20TL50  &    1.020 &    1.393 &    1.672 &    2.061 &    2.254 &    2.318\\ \hline 
T500I0.1P50PL10TL40  &    1.374 &    2.280 &    3.129 &    4.445 &    6.360 &    7.242\\ \hline 
T500I0.4P250PL10TL120  &    0.792 &    1.312 &    1.966 &    3.022 &    4.138 &    5.053\\ \hline 
T500I0.1P100PL20TL50  &    1.028 &    1.848 &    2.343 &    3.730 &    5.404 &    6.253\\ \hline 
T500I0.4P150PL40TL80  &    0.950 &    1.641 &    2.165 &    3.096 &    3.950 &    4.130\\ \hline 
T500I0.1P250PL10TL40  &    0.980 &    1.706 &    2.339 &    3.528 &    4.947 &    5.741\\ \hline 
 Total average  &    1.079 &    1.776 &    2.383 &    3.337 &    4.403 &    5.125\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-33115-pfpmax_eclat.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimipar{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.429 &    2.064 &    3.170 &    2.814 &    3.033 &    2.825\\ \hline 
T500I0.1P50PL20TL40  &    1.426 &    2.298 &    3.457 &    4.414 &    6.078 &    7.625\\ \hline 
T500I0.4P250PL20TL80  &    0.953 &    1.942 &    2.592 &    3.399 &    3.990 &    5.315\\ \hline 
T500I1P100PL20TL50  &    1.107 &    1.369 &    1.840 &    1.687 &    2.209 &    2.082\\ \hline 
T500I0.1P50PL10TL40  &    1.356 &    2.501 &    3.551 &    5.117 &    5.981 &    7.708\\ \hline 
T500I0.4P250PL10TL120  &    0.911 &    1.939 &    2.637 &    3.921 &    5.450 &    5.934\\ \hline 
T500I0.1P100PL20TL50  &    1.096 &    1.959 &    2.711 &    3.916 &    5.364 &    6.242\\ \hline 
T500I0.4P150PL40TL80  &    1.070 &    1.950 &    2.526 &    3.568 &    4.633 &    4.774\\ \hline 
T500I0.1P250PL10TL40  &    1.057 &    2.134 &    2.751 &    3.674 &    5.541 &    6.217\\ \hline 
 Total average  &    1.156 &    2.017 &    2.804 &    3.612 &    4.698 &    5.413\\ \hline 
\end{tabular}


==> tables/avg_speedups/avg_speedup-20000-33115-reservoir.ltx <==
 
\begin{tabular}{|l|l|l|l|l|l|l|}\hline
datafile/\scparfimireserv{} & 2 & 4 & 6 & 10 & 16 & 20\\ \hline
T500I0.4P50PL10TL40  &    1.608 &    2.415 &    3.295 &    3.333 &    5.588 &    6.022\\ \hline 
T500I0.1P50PL20TL40  &    1.423 &    2.381 &    3.029 &    4.046 &    5.472 &    6.304\\ \hline 
T500I0.4P250PL20TL80  &    1.464 &    2.667 &    3.483 &    4.560 &    6.548 &    7.946\\ \hline 
T500I1P100PL20TL50  &    1.190 &    1.876 &    1.862 &    2.528 &    3.838 &    4.414\\ \hline 
T500I0.1P50PL10TL40  &    1.438 &    2.430 &    3.146 &    4.725 &    6.836 &    7.702\\ \hline 
T500I0.4P250PL10TL120  &    1.220 &    2.187 &    3.031 &    4.405 &    6.073 &    6.528\\ \hline 
T500I0.1P100PL20TL50  &    1.146 &    2.040 &    2.227 &    3.705 &    6.315 &    7.501\\ \hline 
T500I0.4P150PL40TL80  &    1.178 &    2.041 &    2.693 &    3.784 &    4.687 &    5.363\\ \hline 
T500I0.1P250PL10TL40  &    1.181 &    2.188 &    2.831 &    4.785 &    6.929 &    7.336\\ \hline 
 Total average  &    1.316 &    2.247 &    2.844 &    3.986 &    5.810 &    6.569\\ \hline 
\end{tabular}

